Understanding Matrix Function Normalizations in Covariance Pooling through the Lens of Riemannian Geometry

Global Covariance Pooling (GCP) has been demonstrated to improve the performance of Deep Neural Networks (DNNs) by exploiting second-order statistics of high-level representations. GCP typically performs classification of the covariance matrices by applying matrix function normalization, such as matrix logarithm or power, followed by a Euclidean classifier. However, covariance matrices inherently lie in a Riemannian manifold, known as the Symmetric Positive Definite (SPD) manifold. The current literature does not provide a satisfactory explanation of why Euclidean classifiers can be applied directly to Riemannian features after the normalization of the matrix power. To mitigate this gap, this paper provides a comprehensive and unified understanding of the matrix logarithm and power from a Riemannian geometry perspective. The underlying mechanism of matrix functions in GCP is interpreted from two perspectives: one based on tangent classifiers (Euclidean classifiers on the tangent space) and the other based on Riemannian classifiers. Via theoretical analysis and empirical validation through extensive experiments on fine-grained and large-scale visual classification datasets, we conclude that the working mechanism of the matrix functions should be attributed to the Riemannian classifiers they implicitly respect. The code is available at https://github.com/GitZH-Chen/RiemGCP.git.

==> Sections/Related_Work.tex <==
\section{Related Work}
\label{sec:related_work}
\textbf{Global covariance pooling.}
GCP aims to leverage the second-order statistics of deep features to enhance the learning competence of DNNs.
$\mathrm{DeepO}^2\mathrm{P}$ \citep{ionescu2015matrix}, acknowledged as the first end-to-end global covariance pooling network, employs matrix logarithm for the classification of covariance matrices.
This method also offers matrix backpropagation to differentiate the gradient w.r.t the decomposition-based matrix functions. 
Following this pioneering work, B-CNN \citep{lin2015bilinear} employs the outer product of global features and carries out element-wise power normalization.
However, there exist three limitations of the above two methods.
Firstly, the high dimensional covariance feature considerably escalates the parameters of the FC layer, thereby introducing the risk of overfitting. 
Secondly, the matrix logarithm could over-stretch the small eigenvalues, undermining the effectiveness of GCP. 
Thirdly, the matrix logarithm is based on matrix decomposition, which is computationally expensive.
The subsequent research primarily focuses on four aspects: (a) adopting richer statistical representation \citep{wang2017g2denet,zheng2019learning,nguyen2021geomnet}; (b) reducing the dimensionality of the covariance feature \citep{gao2016compact,kong2017low,cui2017kernel,acharya2018covariance,rahman2020redro,wang2022dropcov}; (c) investigating effective and efficient matrix normalization \citep{li2018towards,zheng2019learning,lin2017improved,yu2020toward,song2022fasticlr,song2022fast}; (d) improving covariance conditioning for better generalization ability \citep{song2022improving,song2022eigenvalues}. In this work, we do not aim to achieve state-of-the-art performance over the existing GCP-based methods but rather to unravel the underlying theoretical mechanism of GCP matrix functions.

\noindent \textbf{Interpretations of global covariance pooling.}
Along with the progress of GCP, several works began to study its mechanism.
\citet{wang2020gcpoptim} investigate the effect of GCP on deep Convolutional Neural Networks (CNNs) from an optimization perspective, including accelerated convergence, stronger robustness, and good generalization ability.
\citet{wang2023towards} further broaden these investigations, substantiating the merits of GCP in other networks, such as vision transformers \citep{touvron2021training,yuan2021tokens,liu2021swin} and differentiable Neural Architecture Search (NAS) \citep{liu2018darts}.
\citet{song2021approximate} empirically study the advantage of approximate matrix square root over the accurate one.
Wang~\emph{et al.}~\citep{wang2022dropcov} consider the matrix power as decorrelating representations and develop a channel-adaptive dropout to produce lower-dimensional covariance matrices. Nevertheless, existing literature does not fully address the fundamental question of why Euclidean classifiers operate effectively in the non-Euclidean space generated by the matrix power.
Our research fills in this theoretical gap, offering intrinsic explanations regarding the role of the matrix functions in GCP.

\noindent \textbf{Riemannian classifiers on SPD manifolds.}
Since the matrix logarithm is a diffeomorphism between the SPD manifold and its tangent space at the identity \citep{arsigny2005fast}, the most widely used classifier on SPD manifolds is composed of the matrix logarithm and a Euclidean classifier \citep{chen2023adaptive,chen2023riemannian,wang2022dreamnet,wang2021symnet,nguyen2022gyro,nguyen2022gyrovector,wang2022learning,chen2024a}.
However, this tangent classifier might distort the intrinsic geometry of SPD manifolds.
Inspired by HNNs \citep{ganea2018hyperbolic}, recent studies have developed intrinsic classifiers directly on SPD manifolds. 
\citet{nguyen2023building} introduce three gyro structures on SPD manifolds induced by AIM, LEM, and LCM, respectively.
Based on these gyro structures, the authors generalize the Euclidean Multinomial Logistics Regression (MLR).
Concurrently, \citet{chen2024rmlr} propose a formula for SPD MLR under Riemannian metrics pulled back from the Euclidean space.
However, both works require specific Riemannian properties and focus on certain metrics on SPD manifolds.
\citet{chen2024intrinsic} present a general framework for designing Riemannian MLRs on general geometries and showcase their framework under various metrics on SPD manifolds, covering the SPD MLRs introduced in \citep{chen2024rmlr,nguyen2023building}.
In this paper, based on the Riemannian classifiers developed in \citep{chen2024intrinsic}, we present an intrinsic explanation for matrix functions in GCP.






==> link_proof.tex <==
\makeatletter 
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@ 
    \fi
}
\makeatother

\usepackage{etoolbox}
\robustify{\hyperlink}

\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2} 

\makeatother




\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
\newcommand\linkofproof[1]{\newtarget{proof:#1}}
